Generative World Renderer at the Speed of Play

Generative world renderer AlayaRenderer receives structured world states exported from physics engines and synthesizes RGB frames. Unlike models that generate frames from text/control-hints prompts, AlayaRenderer preserves scene structure without altering the underlying world dynamics. This demonstrates an alternative path toward interactive world modeling and user-controllable play. However, the original AlayaRenderer is too computationally expensive for real-time deployment. This technical report introduces AlayaRenderer-Flash, a real-time-oriented generative forward world renderer that pushes AlayaRenderer from 0.56 FPS to 31.54 FPS, reaching the speed of play. AlayaRenderer-Flash reformulates the original renderer as a few-step autoregressive streaming model and introduces lightweight distilled codecs for efficient latent encoding and frame reconstruction. It retains the teacher model's G-buffer and text-prompt interfaces while enabling continuous rendering over input streams of unbounded length. We evaluate AlayaRenderer-Flash on G-buffer streams across content preservation, temporal consistency, cross-window stability, prompt controllability, and runtime efficiency. Our results show that AlayaRenderer-Flash substantially reduces inference cost while preserving the core rendering capabilities of the teacher model. By integrating AlayaRenderer-Flash with a physics engine, we build a fully playable generative world running at 30 FPS.

==> sec/FLUIDdata.tex <==
\section{FLUID Dataset}

The novelty of our \textbf{FLUID dataset} lies in two major aspects:

\begin{enumerate}
    \item \textbf{Closer to realistic interactive scenarios.} 
    Unlike existing datasets (e.g., Meta’s dataset) that mostly simulate two participants engaged in remote, disjoint conversations without physical embodiment, FLUID captures richer and more natural human interactions. In particular, it incorporates \textbf{action-based interactions} and \textbf{action interruptions}, which are critical for modeling dynamic and fluid exchanges in real-world communication.
    
    \item \textbf{Support for multimodal close interaction and 3D reconstruction.}
    Current datasets lack the ability to support 3D reconstruction and do not include physical interactions such as gestures, expressions, or proximity-based behaviors. FLUID is designed as an \textbf{extended version of Harmony4D}, enriched with \textbf{dialogue and close-proximity interactions} between participants. This extension is essential for training AI systems capable of learning \textbf{action- and expression-driven interaction} beyond mere speech exchange.
\end{enumerate}

By introducing these innovations, FLUID provides a unique benchmark for advancing digital humans toward more \textbf{embodied, multimodal, and contextually grounded interaction intelligence}.

